Random-Access Neural Compression of Material Textures

The continuous advancement of photorealism in rendering is accompanied by a growth in texture data and, consequently, increasing storage and memory demands. To address this issue, we propose a novel neural compression technique specifically designed for material textures. We unlock two more levels of detail, i.e., 16x more texels, using low bitrate compression, with image quality that is better than advanced image compression techniques, such as AVIF and JPEG XL. At the same time, our method allows on-demand, real-time decompression with random access similar to block texture compression on GPUs, enabling compression on disk and memory. The key idea behind our approach is compressing multiple material textures and their mipmap chains together, and using a small neural network, that is optimized for each material, to decompress them. Finally, we use a custom training implementation to achieve practical compression speeds, whose performance surpasses that of general frameworks, like PyTorch, by an order of magnitude.

==> inference.tex <==
\section{Inference (Ignore this section: has been merged with Method and Implementation}
\label{sec_inference}
\notetomas{Intro needed here.}

\subsection{Optimization Procedure and Loss Function}
We jointly optimize the texture feature grid pyramid and the decoder together, using stochastic gradient descent.
We use ADAM~\cite{kingma2014adam} optimizer and train the network for 10k-100k iterations, depending on the desired compression speed and quality.

\textbf{TODO describe how we crop and sample mip maps.}

Our method can use and minimize an arbitrary image loss function.
Objective metrics are known to not correspond very well with perceptual
qualities~\cite{blau2018perception}, while perceptual metrics produce \textit{hallucinated} content, similar in image feature statistics, but not corresponding to the original data.
We explored different loss functions for our texture compression algorithm.
\textbf{TODO describe how we tried x/y/z, show a visual comparison of 3-4 and why we decided for L2.}

\begin{figure}[t]
\includegraphics[width=0.9\linewidth, trim=1.5cm 8cm 9cm 0cm, clip]{figures/stochastic_filtering_crop.pdf}
\caption{Bilinear filtering and stochastic filtering.}
\label{fig:fig_stochastic_filter}
\end{figure}
\subsection{Trilinear and Stochastic Filtering}
\notetomas{We need to reference Figure~\ref{fig:fig_stochastic_filter} somewhere.}
GPU texture sampling needs to support filtering on magnification and minification.
Our method provides mip-mapping for discrete levels of minification (Section~\ref{pyramid}), and similarly to BCx compression methods, does not offer other types of filtering in its compressed representation.

The most simple way of applying filtering is to decode and blend multiple texture samples. This can be done in our method, and we have implemented it as a reference.
For the bilinear upsampling, it requires decoding four samples, and eight samples for trilinear interpolation.
This increases the cost of our method (reference to results section), but is similar to how GPUs can provide only lower texture sampling rates on filtration of certain types of textures.

To reduce the computational overhead, we propose another form of filtering, namely, \textit{stochastic filtering}.
\notetomas{It sounds like we introduce stochastic filtering, especially so since there is no reference to any prior work, but stochastically sampling an image is not new. See
https://ieeexplore.ieee.org/document/575247 "A stochastic convolution that describes both image blur and image noise using linear-systems theory", for example. It might
not be the best reference. Perhaps we can reword: "... we suggest using stochastic filtering [ref]."?}
We rely on temporal accumulation (see the survey of ubiquitous temporal super-sampling techniques~\cite{yang2020survey}) to filter the texture over multiple frames.
The only modification to our method is an introduction of stochastic jittering of the sampled position.
We add random noise to the UV position, and by controlling the noise distribution, can produce different types of texture filtering.
For example, uniform distribution in the range $(-1, 1)$ texel extent produces bilinear interpolation, and a normal distribution produces Gaussian interpolation.
After adding noise, we round the UV coordinates to the nearest texel and sample it.
Effectively, this is a form of dithering that selects between different neighboring texels based on the fractional UV coordinates and the noise distribution.
Noise seeds are different each frame and from texel to texel, and temporal accumulation averages multiple samples over a small number of frames.
We note that even in the case of perfect, infinite temporal accumulation, those two methods are not mathematically or practically equivalent.
Traditional PBR material texture filtering averages the individual BRDF properties (between samples created by artists), and our method averages the result of lighting after applying the non-linear rendering process.
\begin{figure}[t]
\includegraphics[keepaspectratio, width=0.9\linewidth]{figures/filtering_comparison_placeholder.png}
\caption{Filtering comparison. \textbf{Left:} Nearest-neighbor filtered reference. \textbf{Middle:} Trilinear material filtering. \textbf{Right:} Our stochastic, temporal filtering.}
\label{fig:fig_filtering_comparison}
\end{figure}
Typical example of an erroneous behavior of PBR texture upsampling is an edge between a dielectric and metal.
Linearly interpolating the metalness (or specularity and diffuse in specularity-based workflow) produces a BRDF that does not correspond to any physical material.
We show a similar example of problematic behavior when a highly specular and matte material cover neighboring texels in Figure~\ref{fig:fig_filtering_comparison}. 
Trilinearly filtering individual PBR properties causes specular lighting artifacts (glossiness interpolation expands the specular outside of the original glossy pixel).

